S$^{2}$FT: Efficient, Scalable and Generalizable LLM Fine-tuning by Structured Sparsity

Current PEFT methods for LLMs can achieve either high quality, efficient training, or scalable serving, but not all three simultaneously. To address this limitation, we investigate sparse fine-tuning and observe a remarkable improvement in generalization ability. Utilizing this key insight, we propose a family of Structured Sparse Fine-Tuning (S$^{2}$FT) methods for LLMs, which concurrently achieve state-of-the-art fine-tuning performance, training efficiency, and inference scalability. S$^{2}$FT accomplishes this by "selecting sparsely and computing densely". It selects a few heads and channels in the MHA and FFN modules for each Transformer block, respectively. Next, it co-permutes weight matrices on both sides of the coupled structures in LLMs to connect the selected components in each layer into a dense submatrix. Finally, S$^{2}$FT performs in-place gradient updates on all submatrices. Through theoretical analysis and empirical results, our method prevents forgetting while simplifying optimization, delivers SOTA performance on both commonsense and arithmetic reasoning with 4.6% and 1.3% average improvements compared to LoRA, and surpasses full FT by 11.5% when generalizing to various domains after instruction tuning. Using our partial backpropagation algorithm, S$^{2}$FT saves training memory up to 3$\times$ and improves latency by 1.5-2.7$\times$ compared to full FT, while delivering an average 10% improvement over LoRA on both metrics. We further demonstrate that the weight updates in S$^{2}$FT can be decoupled into adapters, enabling effective fusion, fast switch, and efficient parallelism for serving multiple fine-tuned models.

==> tables/Data.tex <==
\begin{table}[htbp] 
\centering
\footnotesize
\caption{Details of OOD datasets being evaluated.}
\begin{tabular}{cccc}
\toprule
\textbf{Data} & \textbf{Train}  & \textbf{Validation}& \textbf{Test}\\
% Put SFT results here or leave in ablations
\midrule
\textbf{Flute}  &6659  &120     &749  \\ 
\textbf{GSM}  &7353    & 120    &1319   \\
\textbf{TruthfulQA}  &-    &- &817   \\
\textbf{BBH}  &-   &-           &6511    \\
\textbf{MMLU}  &-   &-          &14042   \\
\textbf{HaluEvalQA}  &-         &10000    \\
\bottomrule
\end{tabular}
\label{tab: data}
\end{table} 

==> tables/OOD_flute.tex <==
\begin{table}[htbp] 
\centering
\footnotesize
\caption{Accuracy comparison of LLaMA2 Chat 7B on OOD benchmarks}
\setlength\tabcolsep{3.0pt} % better format
\begin{tabular}{c|c|c|cccccc|c}
\toprule
\textbf{FT Data} & \textbf{Method}  & \textbf{Param(\%)} & \textbf{Flute} & \textbf{GSM8K} & \textbf{TruthfulQA} & \textbf{BBH} & \textbf{MMLU} & \textbf{HaluEvalQA} & \textbf{Avg. }$\uparrow$ \\
% Put SFT results here or leave in ablations
\midrule
\multirow{7}{*}{Flute} 
&SFT     & 100  & 93.6  & 6.2  & 18.4  & 31.2  &37.9  & 47.1  & 39.1  \\
&L1           & 100  & 94.7  & 16.1  & 25.9  & 38.7  &45.9  & 54.9  & 46.0  \\
&MLP only            & 64.2  & 93.6  & 12.3  & 24.1  & 38.5  & 45.1  & 52.1  & 44.3 \\
&QKV only            & 23.9  & 92.9  & 19.8  & 34.5  & 37.9  & 47.9  & 53.9  & 47.8 \\
&LoRA     & 1.17  & 94.0  & 16.1  & 26.1  & 36.5  & 47.1  & 53.4  & 45.5 \\
&DoRA     & 1.19  & 93.5  & 15.5  & 28.9  & 36.8  & 47.3  & 53.4  & 45.9 \\
&SAU (Ours)   & 1.15  & 94.0  & 23.7  & 35.1  & 38.8  & 47.5  & 53.9  & \textbf{48.8} \\
\midrule
\multirow{7}{*}{GSM8K} 
&SFT     & 100  &  42.5 & 27.1 & 39.3 & 35.8 & 41.2 & 52.4 & 39.7 \\
&L1  & 100  &  49.7 & 29.4 & 39.9 & 36.4 & 44.7 & 52.3 & 42.1 \\
&MLP only  & 64.2  & 47.5 & 25.7 & 36.7 & 36.9 & 40.3 & 53.0 & 40.0 \\
&QKV only  & 23.9  &  49.3 & 33.1 & 39.8 & 38.8 & 47.6 & 52.0 & 43.4 \\
&LoRA     & 1.17  &  50.2 & 30.6 & 38.8 & 37.9 & 45.8 & 52.6 & 42.6\\
&DoRA     & 1.19  &  51.3  & 31.4 & 38.4 & 37.8 & 46.3 & 52.3 & 42.9  \\
&SAU (Ours)   & 1.15  & 54.3 & 32.0 & 38.6 & 39.7 & 47.3 & 52.9 & \textbf{44.1} \\
\bottomrule
\end{tabular}
\label{tab: ood-exp}
\end{table} 
\jxc{DoRA results are still questionable? How are we gonna interpret this (66.8 on flute and 26 on gsm)}

==> text/checklist.tex <==
\section*{NeurIPS Paper Checklist}

\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The abstract and introduction clearly state the contributions of this work.

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{} 
    \item[] Justification: We discuss the limitations of the work in the Conclusion Section (\cref{conclusion}).

\item {\bf Theory Assumptions and Proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerYes{}
    \item[] Justification: The main assumptions and theorems are provided in Section~\ref{sec:theory}, while additional details and complete proofs can be found in Appendix~\ref{app:theory}.
    
\item {\bf Experimental Result Reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{}. % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper has disclosed all the information in the method and experiment part.

\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerNA{}. % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We have the code required to reproduce our experimental results and are working towards making our code available in a public GitHub repository.

\item {\bf Experimental Setting/Details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerYes{}. % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The experimental setting is clearly described in Section~\ref{sec:observation}, Section~\ref{sec:exp} and Section~\ref{sec:efficient}, and we will make our code available in a public GitHub repository.

\item {\bf Experiment Statistical Significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerYes{}. % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification:  All statistics and results included in the paper are accompanied by confidence intervals.

\item {\bf Experiments Compute Resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{}. % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification:  Information for the resources required to reproduce the experiments are included in the oaoer. All experiments are run with 4 x A100 (80G). For the efficiency analysis, a single A100 GPU was used.
    
\item {\bf Code Of Ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{}. % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The research conducted in the paper fully conforms with the NeurIPS Code of Ethics in every respect.


\item {\bf Broader Impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerYes{}. % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We discuss the broader impacts of our work in Appendix.
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{}. % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification:  Our paper does not introduce any assets that have a high risk for misuse.

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{}. % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We have explicitly mentioned the citations for the datasets and have ensured that all conditions are fully respected.

\item {\bf New Assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerNA{}. % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Upon acceptance, we will make our codebase publicly available and complete documentation for our assets.

\item {\bf Crowdsourcing and Research with Human Subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{}. % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We do not include any experiments with human subjects or crowdsourcing.

\item {\bf Institutional Review Board (IRB) Approvals or Equivalent for Research with Human Subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{}. % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We do not include any experiments with human subjects or crowdsourcing.

\end{enumerate}
